Pure competition of multiple species during mixed-substrate microbial growth: Extending the resource-based theory

The simultaneous growth of multiple microbial species is a problem of fundamental ecological interest. In media containing more than one growth-limiting substrate, multiple species can coexist. The question then arises: Can single-species data predict the existence and stability of mixed-culture steady states in mixed-substrate environments? This question has been extensively studied with the help of resource-based models. These studies have shown that the single-species data required to predict mixed-culture behavior consists of the growth isoclines and consumption vectors, which in turn are determined from single-substrate data by making specific assumptions about the kinetics of mixed-substrate growth. Here, we show that these assumptions are not valid for microbial growth on mixtures of substitutable substrates. However, the theory can be developed by determining the growth isoclines and consumption vectors directly from the mixed-substrate data, thus obviating the need for specific assumptions about the kinetics of mixed-substrate growth. We show furthermore that in addition to the growth isoclines and consumption vectors, the single-species, mixed-substrate data yields a new family of curves, which we call the consumption curves. Consideration of the growth isoclines and the consumption curves yields deeper insights into the behavior of the mixed cultures. It yields a priori bounds on the substrate concentrations achieved during coexistence, permits the extension of the theory to systems in which the growth isoclines are non-monotonic, and clarifies earlier results obtained by considering only the growth isoclines.

==> Figures/nontrivial <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 3825 5400 3975 5625
4 0 0 50 0 2 14 0.0000 4 105 90 3825 5550 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3900 5625 2\001
4 0 0 50 0 2 10 0.0000 4 75 60 3900 5475 s\001
-6
6 3825 5625 3975 5850
4 0 0 50 0 2 14 0.0000 4 105 90 3825 5775 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3900 5850 1\001
4 0 0 50 0 2 10 0.0000 4 75 60 3900 5700 s\001
-6
6 3600 2100 3750 2325
4 0 0 50 0 2 14 0.0000 4 105 90 3600 2250 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3675 2325 1\001
4 0 0 50 0 2 10 0.0000 4 75 60 3675 2175 s\001
-6
6 3375 1950 3525 2175
4 0 0 50 0 2 14 0.0000 4 105 90 3375 2100 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3450 2175 2\001
4 0 0 50 0 2 10 0.0000 4 75 60 3450 2025 s\001
-6
6 3375 3975 3525 4200
4 0 0 50 0 2 14 0.0000 4 105 90 3375 4125 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3450 4200 2\001
4 0 0 50 0 2 10 0.0000 4 75 60 3450 4050 s\001
-6
6 3525 4425 3675 4650
4 0 0 50 0 2 14 0.0000 4 105 90 3525 4575 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3600 4650 1\001
4 0 0 50 0 2 10 0.0000 4 75 60 3600 4500 s\001
-6
6 3600 3450 3750 3675
4 0 0 50 0 2 14 0.0000 4 105 90 3600 3600 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3675 3675 1\001
4 0 0 50 0 2 10 0.0000 4 75 60 3675 3525 s\001
-6
6 3600 4800 3750 5025
4 0 0 50 0 2 14 0.0000 4 105 90 3600 4950 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 3675 5025 2\001
4 0 0 50 0 2 10 0.0000 4 75 60 3675 4875 s\001
-6
6 3825 5100 4275 5325
4 0 0 50 0 0 15 0.0000 4 105 90 3825 5325 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 3900 5250 f\001
4 0 0 50 0 0 15 0.0000 4 105 270 3975 5325 - s\001
-6
6 3900 2400 4350 2625
4 0 0 50 0 0 15 0.0000 4 105 90 3900 2625 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 3975 2550 f\001
4 0 0 50 0 0 15 0.0000 4 105 270 4050 2625 - s\001
-6
6 2400 4200 2550 4500
4 0 0 50 0 32 15 0.0000 4 225 90 2400 4425 f\001
4 0 0 50 0 0 10 0.0000 4 105 75 2475 4500 1\001
-6
6 7800 1275 8325 1575
6 7800 1275 8250 1575
6 7875 1275 8025 1575
4 0 0 50 0 0 15 0.0000 4 105 90 7875 1500 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 7950 1425 f\001
4 0 0 50 0 0 10 0.0000 4 105 75 7950 1575 1\001
-6
6 8100 1275 8250 1575
4 0 0 50 0 0 15 0.0000 4 105 90 8100 1500 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 8175 1425 f\001
4 0 0 50 0 0 10 0.0000 4 105 75 8175 1575 1\001
-6
4 0 0 50 0 0 10 0.0000 4 135 60 7800 1500 (\001
-6
4 0 0 50 0 0 10 0.0000 4 45 45 8025 1500 ,\001
4 0 0 50 0 0 10 0.0000 4 135 60 8250 1500 )\001
-6
6 8175 6000 8325 6225
4 0 0 50 0 0 15 0.0000 4 105 90 8175 6150 s\001
4 0 0 50 0 0 10 0.0000 4 105 75 8250 6225 1\001
-6
6 1425 1125 1575 1350
4 0 0 50 0 0 15 0.0000 4 105 90 1425 1275 s\001
4 0 0 50 0 0 10 0.0000 4 105 75 1500 1350 2\001
-6
6 5550 2475 6150 3150
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5616 3134 6141 2834
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5613 3141 6063 2541
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5619 3130 6144 2980
-6
6 6075 2400 6225 2625
4 0 0 50 0 2 14 0.0000 4 105 90 6075 2550 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 6150 2625 2\001
4 0 0 50 0 2 10 0.0000 4 75 60 6150 2475 s\001
-6
6 6075 3150 6225 3375
4 0 0 50 0 2 14 0.0000 4 105 90 6075 3300 r\001
4 0 0 50 0 2 10 0.0000 4 105 75 6150 3375 1\001
4 0 0 50 0 2 10 0.0000 4 75 60 6150 3225 s\001
-6
6 3675 3975 4125 4200
4 0 0 50 0 0 15 0.0000 4 105 90 3675 4200 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 3750 4125 f\001
4 0 0 50 0 0 15 0.0000 4 105 270 3825 4200 - s\001
-6
6 6075 2625 6525 2850
4 0 0 50 0 0 15 0.0000 4 105 90 6075 2850 s\001
4 0 0 50 0 0 10 0.0000 4 105 60 6150 2775 f\001
4 0 0 50 0 0 15 0.0000 4 105 270 6225 2850 - s\001
-6
6 5325 2475 5475 2775
4 0 0 50 0 32 15 0.0000 4 225 90 5325 2700 f\001
4 0 0 50 0 0 10 0.0000 4 105 75 5400 2775 2\001
-6
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 1725 1125 1725 5925 8325 5925
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 1500 3300 5925
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 5025 8100 1650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 3900 8100 1650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 2775 8025 1650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 5775 8100 1650
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 3900 3975 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 4500 3825 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 5025 3825 4650
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 4500 3825 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 4500 3750 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 2775 3450 2175
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 2775 3900 2625
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 5775 3825 5550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 5775 3825 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 5775 3825 5325
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3300 2775 3600 2325
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 4500 8100 1650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 5625 1500 5625 5925
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 4
	 1725 5925 2775 3675 6225 3375 8100 1650
	 0.000 1.000 1.000 0.000
3 0 1 3 0 7 50 0 -1 4.000 0 0 0 5
	 1725 5925 3300 5250 4425 3675 6225 2100 8100 1650
	 0.000 1.000 1.000 1.000 0.000

